Distributed Autoepistemic Logic: Semantics, Complexity, and Applications to Access Control

In this paper we define and study a multi-agent extension of autoepistemic logic (AEL) called distributed autoepistemic logic (dAEL). We define the semantics of dAEL using approximation fixpoint theory, an abstract algebraic framework that unifies different knowledge representation formalisms by describing their semantics as fixpoints of semantic operators. We define 2- and 3-valued semantic operators for dAEL. Using these operators, approximation fixpoint theory allows us to define a class of semantics for dAEL, each based on different intuitions that are well-studied in the context of AEL. We define a mapping from dAEL to AEL and identify the conditions under which the mapping preserves semantics, and furthermore argue that when it does not, the dAEL semantics is more desirable than the AEL-induced semantics since dAEL manages to contain inconsistencies. The development of dAEL has been motivated by an application in the domain of access control. We explain how dAEL can be fruitfully applied to this domain and discuss how well-suited the different semantics are for the application in access control.

==> chapters/daelid.tex <==
\label{sec:daelid}
In this section, we discuss how to extend dAEL with (inductive) definitions (IDs). There are two main reasons for this extension: \begin{enumerate}                                                                                                                                       \item IDs are a common concept in all branches of mathematics; as such, we expect them to be useful as well when reasoning about knowledge
\item in the application 	to access control, the need for IDs arises naturally (see Section \ref{sec:AC}). \end{enumerate}
% We first recall what IDs are and afterwards extend dAEL with them.  

\newcommand{\defs}{\m{\mathit{Def}}}
\renewcommand{\pars}{\m{\mathit{Par}}}
\subsection{Preliminaries: Inductive Definitions}
A definition $\Delta$ over a language $\mc{L}$ is a
set of rules  $\delta$ of the form: $P(\overline{t}) \leftarrow \varphi$ with $\varphi\in \mc{L}$. 
We call $P(\overline{t})$ the head ($head(\delta))$ and $\varphi$ the body ($body(\delta)$) of that rule.
We say that $\Delta$ \emph{defines} $Q$ if $\Delta$ contains a rule $\delta$ with $head(\delta)=  Q(\overline{t})$.
We use $\defs(\Delta)$ to denote all symbols defined in \D; all other symbols are called \emph{parameters}; the set of all parameters is denoted $\pars(\D)$.
% We use $\defs(\Delta)$ and $\pars(\Delta)$ to denote the set of all defined symbols or parameters respectively.  
If $\mc{O}$ is an interpretation of $\pars(\Delta)$ and $I$ a (partial) interpretation of $\defs(\Delta)$, we use $\mc{O}+I$ to interprete symbols in $\pars(\Delta)$ as in $\mc{O}$ and other symbols as in $I$. 
We assume that an interpretation $\mc{O}$ of the parameters is fixed.

AFT defines a family of semantics for inductive definitions  based on a slight generalisation of the immediate consequence operator defined by \citet{jacm/EmdenK76}. 
$T_{\D,\mc{O}}$ maps an interpretation $I$ of $\defs(\Delta) $ to an interpretation $I'$ of $\defs(\Delta) $  such that for defined symbols $P$:
\begin{equation}\label{eq:Tp}
 P(\ddd)^{I'} = \bigor_{\{\delta\in\Delta\mid head(\delta) = P(\ttt)\land \ttt^{I+\mc{O}} = \ddd\}}body(\delta)^{I+\mc{O}}.
\end{equation}

This operator was extended by \citet{Fitting85} for the three-valued setting to an operator $\Psi_{\D,\mc{O}}$, mapping a \emph{partial} $\defs(\Delta)$-interpretation $I$ to a partial $\defs(\Delta)$-interpretation $I'$ such that also Equation \eqref{eq:Tp} holds, now simply replacing two-valued truth valuation by Kleene-valuation. 
% This operator also preserves the value of $I$ on open symbols.


\citetDMT{DeneckerMT00} showed that for each $\mc{O}$, $\Psi_{\D,\mc{O}}$ is an approximator of $T_{\D,\mc{O}}$ and obtained a family of semantics for such definitions. \citet{KR/DeneckerV14} have argued that the well-founded semantics correctly formalises our 
intuition
%intuitive understanding of inductive definitions, 
and hence that it is actually the \emph{right} semantics. Following them, we use the well-founded semantics for IDs; our work can be generalised to allow other semantics for IDs.
Given an interpretation $\mc{O}$ of the parameters of $\D$, we write $w\!f\!m_\Delta(\mc{O})$ for the interpretation $\mc{O}+I$, where $I$ is the $\Psi_{\D,\mc{O}}$-well-founded fixpoint of $T_{\D,\mc{O}}$. 
The well-founded model is also defined if the parameters are only interpreted partially, i.e., in case $\mc{O}$ is a partial interpretation. In this case, $w\!f\!m_\Delta(\mc{O})$ is a partial interpretation as well. 

% \bart{I changed this section quite a bit: made the role of the opens more clear and also renamed them to parameters. The renaming can be undone, but I think the definitions are now more precise}


% \bart{the role of the opens is not very clear yet. Would be better: for each interpretation

\subsection{Syntax and semantics of dAEL(ID)}
dAEL(ID) extends dAEL with modal inductive definitions, where the bodies of rules can contain modal operators. 
We use $\daelid$ as shorthand for this language.
Formally, $\daelid$ consists of logical formulas as in $\dael$ and modal inductive definitions. 
A distributed theory with inductive definitions is an indexed family $\mc{T}=(\T_A)_{A\in\A}$ of theories, i.e.\ sets containing \dael formulas and modal inductive definitions.
The semantics of definitions mainly remains unchanged. All we need to take care of is evaluate modal literals with respect to the distributed belief pair.  As such, we define the immediate consequence (bilattice) operator $\Psi_{\D,\mc{O},\ubp}$ that maps a partial \defs{\D}-interpretation $I$ to $I'$ such that
\[ P(\ddd)^{I'} = \bigor_{\{\delta\in\Delta\mid head(\delta) = P(\ttt)\land \ttt^{I+\mc{O}} = \ddd\}}body(\delta)^{\ubp,I+\mc{O}}.
\]
We write $w\!f\!m_\Delta(\ubp,\mc{O})$ for the (possibly three-valued) $\Psi_{\D,\ubp,\mc{O}}$-well-founded fixpoint.
% $\Delta^\ubp$ is the definition $\Delta$ with all formulas $K\varphi$ replaced by $\Tr$, $\Fa$ or $\Un$, according to their interpretation in $\ubp$.


%We define an immediate consequence operator $\upwsrevisioniddelta$ for $\daelid$ theories, by generalizing \ref{eq:Tp} for modal inductive definitions.
%$\upwsrevisioniddelta$ maps an interpretation $I$ of $\defs(\Delta) $ to an interpretation $I'$ of $\defs(\Delta)$ such that for defined symbols $P$:
%\begin{equation}\label{eq:Tpmodal}
% P(\ddd)^{I'} = \bigor_{\{\delta\in\Delta\mid head(\delta) = P(\ttt)\land \ttt^{I+\mc{O}} = \ddd\}}body(\delta)^{I+\mc{O}+\ubp}.
%\end{equation}
%where $I+\mc{O}+\ubp$ interprets symbols in $\pars(\Delta)$ the same as $\mc{O}$, modal atoms as in $\ubp$ and other symbols the same as $I$.
%Remark that in a partial context ($\ubp$ is three-valued), we cannot yet evaluate the exact value of the defined predicates in the definition. 
%We can, however, using a three-valued valuation of the definition, obtain an approximation $wfm_{\Delta^{\ubp}}(I|_{\pars(\Delta)})$  of their value. 



% \pieter{old:}

We first define a valuation of such definitions with respect to distributed belief pairs (this can also be used for DPWSs). 
\begin{align*}
%&(\Delta)^{\upws,I}=\Tr &&\text{ if } I=wfm_{\Delta^{\upws}}(I|_{\pars(\Delta)}) \\
&\Delta^{\ubp,I}= &&\left\{\begin{array}{ll}
                                  \Tr & \text{ if } I=w\!f\!m_\Delta(\ubp,I|_{\pars(\Delta)}) \\
                                  \Fa & \text{ if } I\not\geq_p w\!f\!m_\Delta(\ubp,I|_{\pars(\Delta)}) \\
                                  \Un & \text{otherwise}
                                 \end{array}\right.
\end{align*}
The intuition here is: \ubp provides partial information about the state of mind of agents. If $I$ is $w\!f\!m_\Delta(\ubp,I|_{\pars(\Delta)})$, then this partial information suffices to determine that the definition is satisfied. Similarly, if $I\not\geq_p w\!f\!m_\Delta(\ubp,I|_{\pars(\Delta)}) $, this information is enough to determine that the definition is not satisfied. Otherwise, the truth of the definition is still unknown (more information on \ubp is needed to determine it). 

% To understand this valuation informally, remark that in a partial context ($\ubp$ is three-valued), we cannot yet evaluate the exact value of the defined predicates in the definition. We can, however, using a three-valued valuation of the definition, obtain an approximation $wfm_{\Delta^{\ubp}}(I|_{\pars(\Delta)})$  of their value. 
% We return $\Tr$ if this approximation is actually $2$-valued and equal to $I$, $\lunkn$ if $I$ is still consistent with (but not equal to) this approximation and $\lfalse$ otherwise. 


% see why this  3-valued valuation (and by consequence the approximator) is correct, assume all modal literals open. %In this case the well-founded of the definition can only become more precise by filling in the opens.
% Note that if in this case the definition has a 2-valued well-founded model, interpreting the opens will never change the value of the definitions (it can only make it more precise).
% As such, independently of the interpretation of the opens $I$ will be the only model satisfying that definition.
% If the well-founded model is 3-valued and $I$ is not more precise than that well-founded model, it follows from the same argumentation that $I$ will not satisfy the definitions for any interpretation of the opens.


The knowledge operator and approximator for $\daelid$ are, using this valuation, simple extensions of those in dAEL.
%e.g.,  
% \begin{definition}\label{def:beliefrevisionupwsid}
% The knowledge revision operator for a $\daelid$ theory $\T$  on a distributed possible world structure $\upws$ is defined as:
% \begin{align*}
% \upwsrevisionid(\upws)&&=(\{I \mid&  \varphi^{\upws,I}=\Tr \text{\quad for each $\varphi \in \T_A$ and}\\ &&&  \Delta^{\upws,I}=\Tr \text{\quad for each ID $\Delta \in \T_A$}\})
% \end{align*}
%\nomenclature{$\upwsrevision(\upws)$}{The knowledge revision operator on a distributed possible world structure.}fjcdjidi
%\end{definition}
The approximation is defined similarly by evaluating all formulas $\varphi$ and definitions $\Delta$ with respect to $\ubp,I$. 



% With this valuation, the definition of the approximator becomes:
% \begin{align*}
% &\ubprevisionidL(\ubp)=(\{I|&& \varphi^{\ubp,I},\Delta^{\ubp,I}=\Tr	  \\ & && \quad \text{for each $\varphi,\Delta \in \T_A$}\})_{A\in \A}\\
% &\ubprevisionidU(\ubp)=(\{I|&& \varphi^{\ubp,I},\Delta^{\ubp,I}\neq\lfalse\\ & && \quad \text{for each $\varphi,\Delta \in \T_A$}\})_{A\in \A}\\
% \end{align*}
% With this valuation, the definition of the approximator is a straightforward extension of the approximator in Section 3.
%

%
%We only need to argue that this is the good valuation. This is not hard: consider all modal literals as opens. 
%These opens are interpreted as in $\ubp$. 
%However, the opens can still be three-valued, which means that we expect the well-founded also to be three-valued. In case it is two-valued, making the opens more precise will never the change the value of the definition. Hence: in this case the %well-founded model is known to be a certain $I$ (true case). 
%In case some $I$ is not more precise than the (three-valued) well-founded model, then it is clear that this $I$ will not satisfy the definition when the opens are made two-valued, so: \lfalse-case. 
%Otherwise, unknown








% 
% \bart{I DONT THINK THAT THE OPERATOR BELOW IS GOOD!!!!  I think it should be: 
% \begin{align*}
% &\ubprevisionidL(\ubp)=(\{I\,|&& \varphi^{\ubp,I}=\Tr \text{\quad for each $\varphi \in \T_A$}\\ & && \quad \text{and } I=wfm_{\Delta^{\ubp}}(I|_{\pars(\Delta)}) \text{ for each}\\ & && \quad \text{definition } \Delta\in \T_A \})_{A\in \A}\\
% &\ubprevisionidU(\ubp)=(\{I\,|&& \varphi^{\ubp,I}\neq \Fa \text{\quad for each $\varphi \in \T_A$}\\ & && \quad \text{and } I\geqp wfm_{\Delta^{\ubp}}(I|_{\pars(\Delta)}) \text{ for each}\\ & && \quad \text{definition } \Delta\in \T_A \})_{A\in \A}
% \end{align*}
% NOTE that we are sometimes replacing formulas by \lunkn in this definition. This is not defined yet above, but is not hard to do it.
% 
% OR EVEN BETTER:
% 
% We can defined $\Delta^{\ubp, I}$, the truth value of a definition wrt an interpretation: 
% \begin{align*}
%  \Delta^{\ubp, I} &= \ltrue &\text{ if } I=wfm_{\Delta^{\ubp}}(I|_{\pars(\Delta)}) \\
%  \Delta^{\ubp, I} &= \lfalse &\text{ if } I\not\geq_p wfm_{\Delta^{\ubp}}(I|_{\pars(\Delta)}) \\
%  \Delta^{\ubp, I} &= \lunkn &\text{ otherwise } 
% \end{align*}
% Then the definition of the operators becomes trivial. 
% We only need to argue that this is the good valuation. This is not hard: consider all modal literals as opens. These opens are interpreted as in $\ubp$. However, the opens can still be three-valued, which means that we expect the well-founded also to be three-valued. In case it is two-valued, making the opens more precise will never the change the value of the definition. Hence: in this case the well-founded model is known to be a certain $I$ (true case). 
% In case some $I$ is not more precise than the (three-valued) well-founded model, then it is clear that this $I$ will not satisfy the definition when the opens are made two-valued, so: \lfalse-case. 
% Otherwise, unknown
% TODO: make text out of this!
% 
% 
% With this valuation, the definition of the operator becomes:
% \begin{align*}
% &\ubprevisionidL(\ubp)=(\{I|&& \varphi^{\ubp,I}=\Tr \text{\quad for each $\varphi \in \T_A$}\\ & && \quad \text{and } \Delta^{\ubp,I}=\Tr \text{ for each}\\ & && \quad \text{definition } \Delta\in \T_A \})_{A\in \A}\\
% &\ubprevisionidU(\ubp)=(\{I|&& \varphi^{\ubp,I}\neq\lfalse\text{\quad for each $\varphi \in \T_A$}\\ & && \quad \text{and } \Delta^{\ubp,I}\neq\lfalse \text{ for each}\\ & && \quad \text{definition } \Delta\in \T_A \})_{A\in \A}\\
% \end{align*}
% }
% 
% 
% \begin{definition}
% Given a distributed belief pair $\ubp$, it is revised with a $\daelid$ theory $\T$ as:
% $$\ubprevisionid(\ubp)=\{\ubprevisionidL(\ubp),\ubprevisionidU(\ubp)\},$$
%  where
% \begin{align*}
% &\ubprevisionidL(\ubp)=(\{I|&& \varphi^{\ubp,I,-}=\Tr \text{\quad for each $\varphi \in \T_A$}\\ & && \quad \text{and } I=wfm_{\Delta^{\ubp^l}}(I) \text{ for each}\\ & && \quad \text{definition } \Delta\in \T_A \})_{A\in \A}\\
% &\ubprevisionidU(\ubp)=(\{I|&& \varphi^{\ubp,I,+}=\Tr \text{\quad for each $\varphi \in \T_A$}\\ & && \quad \text{and } I=wfm_{\Delta^{\ubp^c}}(I) \text{ for each}\\ & && \quad \text{definition } \Delta\in \T_A \})_{A\in \A}
% \end{align*}
% \end{definition}



==> chapters/procedure_old.tex <==
TODO

\todo{first: study complexity of the task ``given a domain D and a theory T'', does this theory entail $K_a\varphi$? Are there other questions we want to study? Give a generic decision procedure?}

\todo{Next: study complexity for fragments? Discuss, e.g., the fragement corresponding to OEL and give decision procedures for fragments?}


\todo{Based on the intro, we might also want to have a ``certified'' task to study. E.g., 
given a sentence $\varphi$ and a theory $T$ and a ``justification'' $J$ for $\varphi$, verify that this is indeed a justification. 
However, that would mean we need some sort of justifications for (d)AEL. }


\subsection{Query-Driven Decision Procedure}\label{sec:query}

We define a query-driven decision procedure for \DACL, which allows to determine access rights while minimizing the information flow between principals in order to enhance security and reduce privacy concerns. This decision procedure is implemented with the help of the \idp system, which we describe in subsection \ref{sec:IDP}. Given that \idp can only work with finite domains, the decision procedure also assumes the domain $D$ to be finite.\footnote{Given that propositional logic has the same expressive power as first-order logic over a finite domain, the decision procedure could in theory also be viewed as a decision procedure for the propositional fragment of \DACL. But since first-order logic over a finite domain can model the same scenarios more concisely and more naturally than propositional logic, we stick to the first-order variant of \DACL with a finite-domain assumption.} For simplicity, we assume that for every principal there is a constant symbol referring to that principal, and that the $t$ in every formula of the form $t \says \phi$ is such a  constant symbol. This simplification could be removed, but would make the description of the decision procedure much more complicated.

The decision procedure is query-driven in the following sense: A query in the form of a \DACL formula $\phi$ is posed to a principal $A$. $A$ determines whether her theory contains enough information in order to verify $\phi$. It can happen that $A$ cannot verify $\phi$ just on the basis of her theory, but can determine that if a certain other principal supports a certain formula, her theory implies the query. For example, $A$'s theory may contain the formula $B \says p \Rightarrow \phi$. In this case, $A$ can forward a remote sub-query to $B$ concerning the status of $p$ in $B$'s theory. If $B$ verifies the sub-query $p$ and informs $A$ about this, $A$ can complete her verification of the original query $\phi$.

% Note that for this communication between the principals about the sub-queries, we assume a certain degree of cooperativity between the principals. This assumption of cooperativity has already been motivated and justified in Subsection \ref{sec:motivation}.

\subsection{Motivation for minimization of information flow}
\label{sec:minimization_motivation}
Consider the following distributed theory of the two principals $A$ and $B$:

\begin{minipage}{0.48\linewidth}
\[ T_A = \left\{
\begin{array}{ll}
   &  r \land B \says s \Rightarrow p  \\
   &  r
\end{array}
 \right\} \]
\end{minipage}~~~~~~~~
\begin{minipage}{0.48\linewidth}
\[ T_B = \left\{
\begin{array}{ll}
   &  s  \\
   &  \neg s \land A \says p \Rightarrow p
\end{array}
 \right\} \]
\end{minipage}
~

In both theories we have a guard, namely, $r$ for theory $T_A$ and $\neg s$ for theory $T_B$. The guards can be checked locally before performing a remote query to other theories. If $A$ is queried about $p$, we can continue with the evaluation and query $T_B$ about the truth value of $s$, since the guard $r$ is true. If $B$ is queried about $p$, on the other hand, we do not need to perform any remote query since it will always fail due to the guard being false in the theory.

If $B$ nevertheless were to send the remote subquery $p$ to $A$, this would be an unnecessary sub-query. Since $B$ does not actually need to know whether $A$ supports $p$, this would violate the need-to-know principle \cite{Sandhu94}, which states that a principal should only be given those accesses and be provided with those non-public informations which the principal requires to carry out her responsibilities. %Assuming that despite their cooperativity, principals do not want their access control policy to be completely public, i.e.\ 
Additionally, it is reasonable to assume that for privacy considerations, the principals do not want to disclose their full access control policies to other principals, but only the parts that are required to verify a given access request. So there are both security and privacy reasons for $B$ not to send the remote subquery $p$ to $A$.

% , it is reasonable to try to fulfill the need-to-know principal in the communication between principals about remote sub-queries needed for evaluating the primary query.

In general, more complex behaviors rather than guards can occur in a distributed theory. The decision procedure we define minimizes the communication even when more complex reasoning is required to determine which sub-queries have a chance of leading to a verification of the primary query and which subqueries are certainly not useful. As discussed in Subsection \ref{sec:complexity}, this ideal minimization of the communication is computationally very expensive, so in a practically applicable system, a trade-off between the security and privacy motivation for minizing communication on the one hand and computational cost on the other hand would need to be found. Nevertheless, we consider our ideal minimization of communication an interesting proof of concept as a foundation for further research.

The decision procedure that determines whether a query $\alpha$ is true given a distributed theory $\T$ is composed of two distinct modules. The first module, the \emph{Query Minimization Procedure}, looks at the theory of the agent to whom the query is directed, and determines minimal sets of remote calls to other theories that could verify the query. The second module, the \emph{Communication Procedure}, takes care of communication between the principals, including the handelling of the loops that may occur.

\subsection{\foid and the \idp-system}\label{sec:IDP}
The decision procedure defined in the next section is based on the \idp system, so we briefly describe this system and its language \foid.

\subsubsection{Why \idp?}

\idp \cite{WarrenBook/DeCatBBD14} is a Knowledge Base System which combines a declarative specification (\emph{knowledge base}), written in an extension of first-order logic, with an imperative management of the specification via the Lua \cite{SPE/IerusalimschyFC96} scripting language. The extension of first-order logic supported by \idp allows for inductive definitions. As explained and motivated in Subsection \ref{sec:motivation}, \DACL also supports inductive definitions. This makes the usage of \idp as a basis for the decision procedure a natural choice. %Inductive definitions can also be (loosely) understood as logic programs in which clause bodies can contain arbitrary first-order formulas. The combination of the declarative specification and the imperative programming environment makes this logic programming tool suitable for solving a large variety of different problems.

\idp supports multiple \emph{inferences} that can be used perform a range of reasoning tasks on a given specification. We make use of two of \idp's inferences, defined in Subsection \ref{sec:foid} below, in order to perform the meta-reasoning about a principal's \DACL theory that is necessary to determine which queries to other principals are really necessary in order to resolve a query asked to the principal.


\subsubsection{\foid and some \idp inferences}
\label{sec:foid}
The specification language supported by \idp is an extension of first-order logic (FO) with types, inductive definitions, aggregates, arithmetic and partial functions, denoted FO(T,ID,Agg,Arit,PF) \cite{KBParadigm16}. We only make use of the subset of FO(T,ID,Agg,Arit,PF) called \foid, which extends FO only with inductive definitions. The formal definition of \foid syntax is the standard definition of FO syntax extended by the following definition of inductive definitions: An \emph{inductive definition} $\Delta$ is a set of rules of the form $\forall \overline{x}:P(\overline{x}) \leftarrow \varphi(\overline{y})$, where $\overline{y} \subset \overline{x}$ and $\varphi(\overline{y})$ is an FO formula. Just as in \DACL, inductive definitions are given the well-founded semantics of inductive definitions \cite{KR/DeneckerV14}. An \foid theory is a set of inductive definitions and FO formulas.

The \idp inferences for \foid that we make use of are defined for \emph{finite partial structures}.
% Given a vocabulary $\Sigma$, a finite partial structure gives an interpretation to (a subset of) the elements of $\Sigma$.
Before we define formally what a partial structure is, we define the concept of a \emph{partial set}, a generalization of a set in a 3-valued context:

\begin{definition}
 A \emph{partial set} on the domain $D$ is a function from $D$ to $\{\Tr,\Fa,\Un\}$, where $\Tr$, $\Fa$ and $\Un$ stand for the three truth-values \emph{true}, \emph{false} and \emph{undefined}.
\end{definition}

A partial set is two-valued (or total) if $\Un$ does not belong to its range.

Given a vocabulary $\Sigma$, a partial structure gives an interpretation to the elements of $\Sigma$:

\begin{definition}
 A \emph{partial structure} over our fixed vocabulary $\Sigma$ is a tuple $(D, \mathcal{I})$, where the domain $D$ is a finite set, and $\mathcal{I}$ is an assignment function that assigns an interpretation to each symbol in $\Sigma$. For a predicate symbol $P$ of arity $n$, the interpretation $P^{\mathcal{I}}$ is a partial set on the domain $D^n$;
%two subsets of $D^n$, denoted as $P^\mathcal{I}_{ct}$ and $P^\mathcal{I}_{cf}$ such that $P^\mathcal{I}_{ct}$ and $P^\mathcal{I}_{cf}$ are disjoint;
for a function symbol $f$ of arity $n$,  $f^\mathcal{I}$ is a function from $D^n$ to $D$.
\end{definition}

When the predicate symbol $P$ has arity $0$, i.e.\ is a propositional variable, $P^{\mathcal{I}}$ is just an element of $\{\Tr,\Fa,\Un\}$.

We call a partial structure $S=(D,\mathcal{I})$ \emph{finite} iff its domain $D$ is finite. We call a partial structure \emph{total} iff $P^\mathcal{I}(\bar{d})$ is total for all $P \in \Sigma, \bar{d} \in D^n$.

The interpretation of terms $t^{\mathcal{I}}$ and the satisfaction relation $\models$ for total structures $S \models \varphi$ are defined as usual.

A precision order can be defined on partial structures:
\begin{definition}
 Given two partial structures $S = (D,\mathcal{I})$ and $S'=(D,\mathcal{I}')$, we write $S \leq_p S'$ (and say $S$ \emph{is more precise than} $S'$, or $S'$ \emph{expands} $S$) iff for every function symbol $f$, $f^{\mathcal{I}'} = f^\mathcal{I}$, and for every predicate symbol $P$ of arity $n$ and every tuple $\bar d \in D^n$ of domain elements such that $P^\mathcal{I}(\bar d) \neq \Un$, we have $P^{\mathcal{I}'}(\bar d) = P^\mathcal{I}(\bar d)$.
\end{definition}

We now define the two \idp inferences that we make use of. The first one, which is called \texttt{sat} in the \idp system, determines whether a given finite partial structure is a partial model of a given theory:

\begin{definition} Let $S$ be a partial structure and $\mathcal{T}$ an \foid theory. We say $S$ is a \emph{partial model} for $\mathcal{T}$ if and only if there exists a total structure $S^\prime \geq_p S$ such that $S^\prime \models \mathcal{T}$.
\end{definition}

The second \idp inference that we make use of, which is called \texttt{unsatstructure} in the \idp system, picks a minimal partial structure inconsistent with a given theory and less precise than a given finite partial structure:

\begin{definition} Let $S$ be a partial structure and $\mathcal{T}$ be an \foid theory. We define $min\_incons\_set(\mathcal{T},S)$ to be the set of $\leq_p$-minimal partial structures $S^\prime \leq_p S$ such that $S^\prime$ is not a partial model of $\mathcal{T}$ has no models that expand $S$.
% We define $min\_incons(\mathcal{T},S)$ to be the lexicographically first structure in $min\_incons\_set(\mathcal{T},S)$.
\end{definition}

If the input structure $S$ is not a partial model of the input structure $\mathcal{T}$, $min\_incons\_set(\mathcal{T},S)$ is always non-empty, and \texttt{unsatstructure} picks an element from it and returns it. If $S$ is a partial model of $\mathcal{T}$ \texttt{unsatstructure} throws an error.


\subsection{Query Minimization Procedure}

\subsubsection{Translation Mechanism}

In order to implement a query mechanism for \DACL in IDP we need to translate \DACL theories to \foid theories.
The only syntactic construct of \DACL that does not exist in \foid is the \say-modality. So when translating a \DACL theory $T$ to an \foid theory $\mathcal{T}$, we need to replace each \say-atoms in $T$ by some first-order formula. For this purpose, we extend the vocabulary $\Sigma$ to an extended vocabulary $\Sigma'$ by adding to it new propositional variables of the form $p^+_{A\_{\verb=says=\_\varphi}}$, $p^-_{A\_{\verb=says=\_\varphi}}$ and $w_{A\_{\verb=says=\_\phi}}$ for every modal statement $A \says \varphi$ of \DACL.

Before we formally define the translation mechanism, let us first motivate why we have the three different propositional variables $p^+_{A\_{\verb=says=\_\varphi}}$, $p^-_{A\_{\verb=says=\_\varphi}}$ and $w_{A\_{\verb=says=\_\phi}}$ for translating different occurrences of the same \say-atom $A \says \phi$. First, note that the well-founded semantics of \DACL evaluates \say-atoms in a three-valued way. The propositional variables $p^+_{A\_{\verb=says=\_\varphi}}$ and $p^-_{A\_{\verb=says=\_\varphi}}$ are used to model the three-valued valuation of $A \says \phi$ in the two-valued logic \foid: On the precision order $<_p$ on the three truth values $\ltrue$ (\emph{true}), $\lfalse$ (\emph{false}) and $\lunkn$ (\emph{undefined})
induced by $\lunkn<_p\ltrue$ and $\lunkn<_p\lfalse$, the propositional variable $p^+_{A\_{\verb=says=\_\varphi}}$ represents the upper bound for the truth value of $A \says \varphi$ and $p^-_{A\_{\verb=says=\_\varphi}}$ the lower bound. For this reason, we replace every positive occurrence of $A \says \phi$ by $p^+_{A\_{\verb=says=\_\varphi}}$, and every negative occurrence by $p^-_{A\_{\verb=says=\_\varphi}}$. Given that occurrences of a formula in an inductive definition cannot be meaningfully termed only positive or only negative, we first replace occurrences of $A \says \phi$ in an inductive definition by $w_{A\_{\verb=says=\_\phi}}$ and add two implications to the theories that express the equivalence between $w_{A\_{\verb=says=\_\psi}}$ and $A \says \phi$.

The translation function $t$ only performs this first step of the translation mechanism:

\begin{definition}Let $T$ be a \DACL theory. We define $t(T)$ to be a \DACL theory equivalent to $T$, constructed as follows:

For every modal atom $A \says \varphi$ occurring in the body of an inductive definition in theory $T$,
\begin{itemize}
  \item  replace $A \says \varphi$ by the propositional variable $w_{A\_{\verb=says=\_\varphi}}$
  \item  add to $t(T)$ the two formulae $w_{A\_{\verb=says=\_\varphi}} \Rightarrow A \says \varphi$ and $A \says \varphi \Rightarrow w_{A\_{\verb=says=\_\varphi}}$.
\end{itemize}
\end{definition}


We next introduce the notion of polarity necessary to further translate \DACL theories into \foid theories. 


\begin{definition} Let $\phi$ be a \DACL formula. The \emph{polarity} of an occurrence of a subformula of $\phi$ is defined recursively as follows:
\begin{itemize}
\item The occurrence of $\phi$ in $\phi$ is a \emph{positive} occurrence.
\item Given a positive (resp. \emph{negative}) occurrence of the the subformula $\neg \psi$ of $\phi$, the occurence of $\psi$ in this occurrence of $\neg \psi$ is \emph{negative} (resp. \emph{positive}) in $\phi$.
%\item[iii-] If $\psi \lor \chi$ is a \emph{positive} (resp. \emph{negative}) sub-formula of $\phi$, then $\psi$ and $\chi$ are both \emph{positive} (resp. \emph{negative}) sub-formulas of $\phi$.
\item Given a \emph{positive} (resp. \emph{negative}) occurrence of the subformula $\psi \land \chi$ of $\phi$, the occurrences of $\psi$ and $\chi$ in this occurrence of $\psi \land \chi$ are both \emph{positive} (resp. \emph{negative}) in $\phi$.
%\item[v-] If $\psi \to \chi$ is a \emph{positive} (resp. \emph{negative}) sub-formula of $\phi$, then $\psi$ is a \emph{negative} (resp. \emph{positive}) sub-formula and $\chi$ is a \emph{positive} (resp. \emph{negative}) sub-formula of $\phi$.
%\item[vi-] If $\psi \leftrightarrow \chi$ is a sub-formula of $\phi$, then every sub-formula of $\psi$ and $\chi$ is positive and negative sub-formula of $\phi$.
\end{itemize}
\end{definition}

\begin{definition}
 Let $T$ be a \DACL theory, let $\phi \in T$. We call a positive (resp. negative) occurrence of a subformula $\psi$ of $\phi$ a \emph{positive} (resp. \emph{negative}) \emph{occurrence} of $\psi$ in $T$.
\end{definition}


Now we can define the translation function $\tau$ from \DACL theories to \foid theories:

\begin{definition} Let $T$ be a \DACL theory. $\tau(T)$ is constructed from $t(T)$ by performing the following replacements for every \say-atom $A \says \varphi$ occurring in $t(T)$ that is not the subformula of another \say-atom:
\begin{itemize}
  \item Replace every positive occurrence of $A \says \varphi$ in $T$ by $p^+_{A\_{\verb=says=\_\varphi}}$.
  \item Replace every negative occurrence of $A \says \varphi$ in $T$ by $p^-_{A\_{\verb=says=\_\varphi}}$.
\end{itemize}
\end{definition}

We will illustrate the translation procedure with a simple example, which we will use as a running example to be extended throughout the section.

\begin{example}\label{ex:example} Let $\A=\{A,B,C\}$, and let the distributed theory $\T$ consist of the folowing three \DACL theories:

\begin{minipage}{0.48\linewidth}
  \[ T_A = \left\{
\begin{array}{ll}
   &  \{ \ p \leftarrow B ~\says~ p,  \\
   & p \leftarrow r \ \} \\
   &  p \land s \land B ~\says~ z \Rightarrow z \\
   & r \lor \neg r \Rightarrow s\\
   & B ~\says~ r \lor \neg (B ~\says~ r) \Rightarrow z
\end{array}
 \right\} \]
\end{minipage} \hfill
\begin{minipage}{0.48\linewidth}
\[ T_B = \left\{
\begin{array}{ll}
   &  p  \\
   &  C ~\says~ z \Rightarrow z \\
   & C ~\says~ r \Rightarrow r
\end{array}
 \right\} \]
\[ T_C = \left\{
\begin{array}{ll}
   &  \neg(B ~\says~ z) \Rightarrow z  \\
   &  B ~\says~ r \Rightarrow r
\end{array}
 \right\} \]
\end{minipage}
~

We translate these theories as follows:

\begin{minipage}{0.48\linewidth}
\[ \tau(T_A) = \left\{
\begin{array}{ll}
& \{ \ p \leftarrow w_{B\_{\texttt{says}\_p}},	\\
& p \leftarrow r \ \} \\
& w_{B\_{\texttt{says}\_p}} \Rightarrow p^+_{B\_{\texttt{says}\_p}}\\
& p^-_{B\_{\texttt{says}\_p}} \Rightarrow w_{B\_{\texttt{says}\_p}}\\
& p \land s \land p^-_{B\_{\texttt{says}\_z}} \Rightarrow z\\
& r \lor \neg r \Rightarrow s\\
& p^-_{B\_{\texttt{says}\_r}} \lor \neg p^+_{B\_{\texttt{says}\_r}} \Rightarrow z\\
%& p^-_{B\_{\texttt{says}\_p}} \to p^+_{B\_{\texttt{says}\_p}}\\
%& p^-_{B\_{\texttt{says}\_r}} \to p^+_{B\_{\texttt{says}\_r}}
\end{array}
 \right\} \]
\end{minipage}
\begin{minipage}{0.48\linewidth}
\[ \tau(T_B) = \left\{
\begin{array}{ll}
& p\\
& p^-_{C\_{\texttt{says}\_z}} \Rightarrow z \\
& p^-_{C\_{\texttt{says}\_r}} \Rightarrow r
\end{array}
 \right\} \]
\[ \tau(T_C) = \left\{
\begin{array}{ll}
& \neg p^+_{B\_{\texttt{says}\_z}} \Rightarrow z\\
& p^-_{B\_{\texttt{says}\_r}} \Rightarrow r
\end{array}
 \right\} \]
\end{minipage}
\end{example}

~
\subsubsection{Query Minimization Procedure} \label{subsec:minimization}


The query minimization procedure works as follows: given a theory $T$ and a query $\alpha$, the procedure returns a set $\mathbb{L}$ of sets of modal atoms. The intended meaning of $\mathbb{L}$ is as follows: When all modal atoms in a set $L \in \mathbb{L}$ can be determined to be true, the query $\alpha$ succeeds, and $\mathbb{L}$ is the set of all sets $L$ with this property. This means that if $\mathbb{L} = \emptyset$, the query necessarily fails, whereas if $\mathbb{L}$ contains $\emptyset$, the query necessarily succeeds.

A partial structure $S$ over the extended vocabulary $\Sigma'$ contains information about the truth values of the propositional variables of the form $p^-_{A\_{\verb=says=\_\varphi}}$ and $p^+_{A\_{\verb=says=\_\varphi}}$. Taking into account that $p^-_{A\_{\verb=says=\_\varphi}}$ and $p^+_{A\_{\verb=says=\_\varphi}}$ are used to represent the three-valued valuation of $A \says \phi$, this information can also be represented by a set of \say-literals, which we denote $L^S$:

\begin{definition} For a partial structure $S=(D,\mathcal{I})$, we define $L^S$ to be 
$$\{A \says \varphi \;|\; (p^-_{A\_{\verb=says=\_\varphi}})^\mathcal{I} = \Tr\} \cup  \{\neg A \says \varphi \;|\; (p^+_{A\_{\verb=says=\_\varphi}})^\mathcal{I} = \Fa\}$$
\end{definition}

We say that a \say-atom $A \says \phi$ \emph{occurs directly} in a \DACL theory, if some occurrence of $A \says \phi$ in $\T$ is not a subformula of another \say-atom. In the Query Minimization Procedure, we need to take into account all possible three-valued valuations of the \say-atoms directly occurring in the input \DACL theory $T$. Such a valuation can be represented by a partial structure that contains information only about propositional variables of the form $p^+_{A\_\texttt{says}\_\varphi}$ and $S \models p^-_{A\_\texttt{says}\_\phi}$, and for which this information is coherent in the sense that the truth values assigned to $p^+_{A\_\texttt{says}\_\varphi}$ and $S \models p^-_{A\_\texttt{says}\_\phi}$ are compatible. This is made formally precise in the following definition of the set $\mathbb{S}_T$ that contains all structures that represent three-valued valuations of \say-atoms directly occurring in $T$:

\begin{definition} Let $T$ be a \DACL theory. We define $\mathbb{S}_T$ to be the set containing every partial structure $S=(D,\mathcal{I})$ over vocabulary $\Sigma'$ satisfying the following properties:
\begin{itemize}
 \item $P^{\mathcal{I}^S} = \mathbf{u}$ for every symbol in $\Sigma'$ that is not of the form $p^+_{A\_\texttt{says}\_\varphi}$ or $p^-_{A\_\texttt{says}\_\phi}$ for some \say-atom $A \says \varphi$ occurring in $\tau(T)$.
 \item For every \say-atom $A \says \phi$, $(p^+_{A\_\texttt{says}\_\varphi})^\mathcal{I} \neq \Tr$.
 \item For every \say-atom $A \says \phi$,  $(p^-_{A\_\texttt{says}\_\varphi})^\mathcal{I} \neq \Fa$.
 \item For no \say-atom $A \says \phi$, $(p^+_{A\_\texttt{says}\_\varphi})^\mathcal{I} = \Fa$ and $(p^-_{A\_\texttt{says}\_\varphi})^\mathcal{I} = \Tr$.
\end{itemize}
\end{definition}

We are now ready to define the Query Minimization Procedure. Its pseudo-code is as follows (Algorithm 1). Please note that lines 4 and 5 are implemented using the \idp inferences \texttt{sat} and \texttt{unsatstructure} that we defined in Section \ref{sec:foid}.

\begin{algorithm}[h!t]
\caption{\textsf{Query Minimization Procedure} \label{alg:query}}
\begin{algorithmic}[1]
\REQUIRE{theory $T$, \DACL query $\alpha$ }
\ENSURE{set $\mathbb{L}$ of sets of modal atoms}
    \STATE{$\mathbb{L}$ := $\emptyset$ }
    \STATE{$\mathcal{T}$ := $\tau(T)$ }
\FOR{ \textbf{each} $S \in  \mathbb{S}_T$}
      \IF{ $S$ is not a partial model of $\mathcal{T} \cup \{\neg \alpha\}$}
        \STATE{pick a partial structure $S_{min}$ from $min\_incons\_set(\mathcal{T} \cup \{ \neg \alpha \},S)$}
        \STATE{ $\mathbb{L}$ := $\mathbb{L} \cup \{L^{S_{min}}\}$ }\label{lin:last}
    \ENDIF
\ENDFOR
\RETURN{$\mathbb{L}$}
\end{algorithmic}
\end{algorithm}
~

The algorithm is to be read as follows. A query $\alpha$ asked to theory $T$ is given as input. First (line 2) we 
translate $T$ to the \foid theory $\mathcal{T}=\tau(T)$. Next we iterate over the structures $S \in \mathbb{S}_T$ (lines 3-6).
Line 4 ensures that we limit ourselves to structures $S \in \mathbb{S}_T$ that are not a partial models of $\mathcal{T} \cup \{\neg \alpha\}$; note that the information in such a structure $S$ together with the information in $\mathcal{T}$ entails the query $\alpha$. 
Furthermore, note that for such a structure $S$, $min\_incons\_set(\mathcal{T} \cup \{ \neg \alpha \},S)$ is non-empty. So next (line 5), we pick a structure $S_{min}$ from $min\_incons\_set(\mathcal{T} \cup \{ \neg \alpha \},S)$; by definition $S_{min}$ is a minimal structure such that $S_{min} \leq_p S$ and $S_{min}$ is not a partial model of $\mathcal{T} \cup \{\neg \alpha\}$; this means that $S_{min}$ contains a minimal amount of information from $S$ that together with the information in $\mathcal{T}$ ensures the query $\alpha$ to be true. So the set $L^{S_{min}}$, which represents the same information as a set of \say-literals, is a minimal set of \say-literals that together with the information in $T$ ensure the query $\alpha$ to be true.\footnote{Lemma \ref{lem:minimization} in Appendix B makes this claim more precise.}
Line 6 adds $L^{S_{min}}$ to the set of sets of \say-literals that we output at the end (line 7), after the iteration over the elements of $\mathbb{S}_T$ is completed.




We continue Example \ref{ex:example} to illustrate the query minimization procedure.

\begin{example} \label{ex:query-min} We apply the Query Minimization Procedure to the theory $T_A$ and the query $z$.
First we translate the theory $T_A$ to $\mathcal{T} = \tau(T_A)$, which we have shown in Example \ref{ex:example}.
Then we iterate over the structures $S \in \mathbb{S}_{T_A}$.

Let, for example, $S$ be the element of $\mathbb{S}_{T_A}$ that makes $p^-_{B\_{\texttt{says}\_p}}$ and $p^-_{B\_{\texttt{says}\_r}}$ true and everything else undefined. Then $S$ is a not partial model of $\mathcal{T} \cup \{\neg z\}$, because $p^-_{B\_{\texttt{says}\_p}}$ is inconsistent with $p^-_{B\_{\texttt{says}\_r}} \lor \neg p^+_{B\_{\texttt{says}\_r}} \Rightarrow z$ and $z$. Now $min\_incons\_set(\mathcal{T} \cup \{ \neg z \},S)$ is the set consisting only of the structure $S'$ that makes $p^-_{B\_{\texttt{says}\_p}}$ true and everyting else undefined. So in line 5, we necessarily pick $S_{min}$ to be this structure $S'$. In line 6 we calculate $L^{S'}$ to be $\{B \says r\}$ and add $\{B \says r\}$ to $\mathbb{L}$.


When we iterate over all structures $S \in \mathbb{S}_{T_A}$, the value of $\mathbb{L}$ finally becomes 
$$\{\{B \says r\}, \{B \says p, \\ B \says z\},\{\neg B \says r\}\}.$$
\end{example}



\subsection{Communication and loop handling}

In this subsection we describe the Communication Procedure, which also takes care of the loop-handling. The Communication Procedure calls the Query Minimization Procedure and thereby constitutes our decision procedure for \DACL.

When a query is asked to a principal, the Query Minimization Procedure determines minimal sets of \say-literals that need to be satisfied in order to verify the query. The Communication Procedure then produces remote sub-queries to other principals that can determine the status of the \say-literals.

The Communication Procedure works by dynamically producing a \emph{query graph} and attaching three-valued truth values to the query vertices in it:

\begin{definition}
\label{def:query graph}
A \emph{query graph} is a labelled directed graph with two kinds of vertices and two kinds of edges:
 \begin{itemize}
  \item The first kind of vertices are the \emph{query vertices}. Each query vertex is labelled by a directed query of the form $\langle k:\phi \rangle$, where $k$ is the principal whose theory is being queried and $\phi$ is the formula representing the query. Additionally, a query vertex is potentially labelled by a truth value in $\{\Tr,\Fa,\Un\}$, which represents the currently active valuation of the query at any moment during the execution of the decision procedure.
  \item The second kind of vertices are the \emph{\say-literal set vertices}. Each \say-literal set vertex is labelled by a set of \say-literals, i.e.\ formulas of the form $k \says \phi$ or $\neg k \says \phi$.
  \item The first kind of edges are unlabelled edges going from a query vertex to a \say-literal set vertex. The intended meaning of such an unlabelled edge from $\langle k:\Q \rangle$ to the \say-literal set $L$ is that one way of making $\Q$ true in $k$'s theory is to make all \say-literals in $L$ true.
  \item The second kind of edged are edges labelled by $\Tr$ or $\Fa$, going from a \say-literal set vertex to a query vertex. The intended meaning of such an edge labelled by $\Tr$ or $\Fa$ and going from the \say-literal set $L$ to the query $\langle k:\Q \rangle$ is that $L$ contains the literal $ k \says \Q $ or the literal $\neg k \says \Q$ respectively.
 \end{itemize}
\end{definition}

The query graphs are actually always trees, with the query vertex corresponding to the original query as their root. %The reason why we define

The Communication Procedure starts with a query graph consisting just of the query vertex $\langle A:\alpha \rangle$, where $A$ is the principal to whom the primary query $\alpha$ is asked. Next the Communication Procedure calls the Query Minimization Procedure to add sub-queries to the query graph and attach truth values to them. This procedure is iteratively continued until a truth-value has been attached to the root vertex $\langle A:\alpha \rangle$.

The Communication Procedure is defined via an initialization procedure defined under Algorithm \ref{alg:init}, which calls the main recursive procedure defined under Algorithm \ref{alg:comm}.

\begin{algorithm}[h!t]
\caption{\textsf{Communication Procedure Initialization} \label{alg:init}}
\begin{algorithmic}[1]
\REQUIRE{distributed theory $\T$, principal $A$, \DACL formula $\Q$}
\ENSURE{truth-value $V \in \{\Tr,\Fa,\Un\}$}
\STATE{$G$ := the labelled graph consisting only of a single vertex $v$ labelled $\langle A:\Q \rangle$ and no edges }
% \STATE{add a new query vertex $v$ labelled $A:\Q$ to $G$}
% \STATE{$k$ := $A$}
% \STATE{$\phi$ := $\Q$}
\STATE{$G$ := Communication\_{}Procedure($\T$,$G$,$v$)}
\STATE{$V$ := the label on the query vertex $\langle A:\Q \rangle$ in $G$}
\RETURN{$V$}
\end{algorithmic}
\end{algorithm}

Informally, the Communication Procedure can be explained as follows: The Query Minimization Procedure is called for $\T_A$ and $\alpha$. It returns a set of sets of \say-literals. For each such \say-literal set, we add a \say-literal set vertex connected to the root query vertex $\langle A:\alpha \rangle$ (lines 6-7). For each \say-literal in this set, we add a query vertex and an edge from the set vertex to this query vertex labelled by $\Tr$ or $\Fa$ depending on the sign of the \say-literal (8-15). We then apply Query Minimization Procedure and the rest of the procedure just explained to each new query vertex (line 22). At the same time, we label query vertices with truth values as follows: When all query vertices emerging from a \say-literal set vertex are labelled with the same truth value as the edge through which they are connected to the \say-literal set vertex, the query that produced that \say-literal set vertex is labelled $\Tr$ (lines 23-24). There is a dual procedure for labelling query vertices with $\Fa$ (lines 25-26). When a loop is detected, the query vertex causing the loop (by having the same label as a query vertex that is an ancestor of it) is labelled either with $\Fa$ or $\Un$, depending on whether the loop is over a negation (i.e. there is an $\Fa$-labelled edge in the path connecting the two vertices with the same label) or not (lines 16-20). $\Un$-labels  can also propagate towards the root of the graph (line 28).

\begin{algorithm}[h!t]
\caption{\textsf{Communication Procedure} \label{alg:comm}}
\begin{algorithmic}[1]
\REQUIRE{distributed theory $\T$, query graph $G$, query vertex $v$ of $G$,}
\ENSURE{updated query graph $G$}
\STATE{$k$ := the principal mentioned in the label of $v$}
\STATE{$\phi$ := the formula mentioned in the label of $v$}
\STATE{$\LL$ := \textsf{Query\_{}Minimization\_{}Procedure}($\T_k$,$\phi$)}
\WHILE{the input query vertex $v$ does not have a truth-value attached to it}
  \FOR{$L \in \LL$}
    \STATE{add a new \say-literal set vertex $L$ to $G$}
    \STATE{add to $G$ a new edge from vertex $v$ to vertex $L$}
%     \WHILE{there is no edge labelled $\Tr$ from set vertex $L$ to a query vertex labelled $\Tr$}
      \FOR{$l \in L$}
        \STATE{$k'$ := the principal such that $l$ is of the form $k' \says \psi$ or $\neg k' \says \psi$}
        \STATE{$\psi$ := the formula such that $l$ is of the form $k' \says \psi$ or $\neg k' \says \psi$}
        \STATE{add a query vertex $v'$ labelled by $\langle k':\psi \rangle$ to $G$}
        \IF{$l$ is $k' \says \psi$}
          \STATE{add to $G$ a new edge labelled $\Tr$ from vertex $L$ to vertex $\langle k':\psi \rangle$}
        \ENDIF
        \IF{$l$ is $\neg k' \says \psi$}
          \STATE{add to $G$ a new edge labelled $\Fa$ from vertex $L$ to vertex $\langle k':\psi \rangle$}
        \ENDIF
        \IF{a query vertex $v''$ that is an ancestor of $v'$ is also labelled $\langle k':\psi \rangle$}
          \IF{all labelled edges between $v''$ and $v'$ are labelled by $\Tr$}
            \STATE{add $\Fa$-label to $v'$}
          \ELSE
	    \STATE{add $\Un$-label to $v'$}
          \ENDIF
        \ELSE
	  \STATE{Communication\_{}Procedure($\T$,$G$,$v'$)}
        \ENDIF
      \ENDFOR
%     \ENDWHILE
      \IF{every query vertex $v'$ such that there is an edge from $L$ to $v'$ is labelled with the same truth value as this edge}
        \STATE{label $v$ with $\Tr$}
      \ENDIF
  \ENDFOR
  \IF{for every \say literal set vertex $L$ such that there is an edge from $v$ to $L$, there is a query vertex $v'$ such that there is an edge from $L$ to $v'$ labelled with the opposite truth value as $v'$}
    \STATE{label $v$ with $\Fa$}
  \ELSE
    \STATE{label $v$ with $\Un$}
  \ENDIF
\ENDWHILE
\RETURN{$G$}
\end{algorithmic}
\end{algorithm}


We continue Example \ref{ex:example} to illustrate the Communication Procedure.

\begin{example} Given the distributed theory $\T = \{T_A, T_B, T_C\}$, we query the principal $A$ about the truth value of $z$. We show the final graph in Figure \ref{fig:graph} and now explain its construction.
We start by calling the Communication Initialization Procedure; this generates a graph $G$ with the vertex $v =\langle A:z \rangle$  (with no associated truth value label). Then we call the Communication Procedure with arguments $\T$, $G$ and $v$.
We call the Query Minimization Procedure returning the set $\mathbb{L} = \{\{B \says p, B \says z\}, \{B \says r\}, \{\neg B \says r\}\}$ as shown in Example \ref{ex:query-min}. Since the input vertex $v$ has no truth-value associated to it, we next iterate over the sets $L \in \mathbb{L}$.
The \say-literal set vertex $\{B \says p, B \says z\}$ is added to $G$ with its corresponding edge.
Now we consider each \say-literal in the vertex. 

(i) For literal $B \says p$ generate a new query vertex $v^\prime = \langle B: p \rangle$ with an edge labelled $\mathbf{t}$ (since the literal is not negated) and recursively call the Communication Procedure with the updated graph as argument and vertex $v^\prime$. $v^\prime$ has no truth-value associated, the Query Minimization Procedure returns the set $\mathbb{L}^\prime = \{\{\}\}$; so after adding the \say-literal set vertex $\{\}$ connected to $v^\prime$, the truth-value $\mathbf{t}$ is assigned to $v^\prime$ by lines 21-22 of the Communication Procedure (this corresponds to the intuitive idea that $\mathbb{L}^\prime = \{\{\}\}$ means that $p$ is true in $T_B$).

(ii) For literal $B \says z$ generate a new query vertex $v^\prime = \langle B: z \rangle$ with an edge labelled $\mathbf{t}$ and recursively call the Communication Procedure with the updated graph as argument and vertex $v^\prime$. The Query Minimization Procedure is called returning the set $\mathbb{L} = \{\{C \says z\}\}$; for this literal we generate a new query vertex $v^{\prime\prime} = \langle C: z \rangle$ with an edge labelled $\mathbf{t}$. In turn, the Query Minimization Procedure is called returning the set $\mathbb{L}^{\prime\prime}= \{\{\neg B \says z\}\}$; for this literal we generate a new query vertex $v^{\prime\prime\prime} = \langle B: z \rangle$ with an edge labelled $\mathbf{f}$. 
At this point we detect a loop, as the query vertex $v^\prime$ that is an ancestor of $v^{\prime\prime\prime}$ is also labelled by $\langle B: z \rangle$. Since the loop contains an edge with label $\mathbf{f}$, the truth-value assignment for $v^{\prime\prime\prime}$ is  $\mathbf{u}$. This truth-value $\mathbf{u}$ is propagated up to label the query vertices $v^{\prime\prime}$ and $v^{\prime}$, since $\mathbf{u}$ does not match with either $\mathbf{t}$ nor $\mathbf{f}$.

Finally, the truth-values for (i) matches the labeled edge, but not for the case of (ii). Thus we cannot yet label the root vertex with $\Tr$, and continue with the next \say-literal $\{B \says r\} \in \mathbb{L}$.

For vertex $\{B \says r\}$, we repeat the procedure as described above until we (again) detect a loop. This loop does not contain edges with label $\mathbf{f}$, so the truth-value assignment for the vertex at which the loop is detected is $\mathbf{f}$.
Again this truth-value is propagated to label the two query vertices above this vertex, as the labelled edges are labelled by $\mathbf{t}$. Since the truth-value $\Fa$ assigned to the query vertex $\langle B:r\rangle$ does not match the truth value of the labelled edge above it, the root vertex can still not be labelled with $\Tr$.

The subgraph produced below the final \say-literal set vertex $\{\neg B \says r\}$ is the same as below \say-literal set vertex $\{B \says r\}$, only that the labelled edge directly below this \say-literal set vertex is now labelled $\Fa$ instead of $\Tr$. So this time the label on the query vertex $\langle B:r\rangle$ matches the label on the labelled edge, to that the root vertex is labelled $\Tr$. This ends the main while loop and therefore the Communication Procedure. Finally, the Communication Procedure Initialization returns the output $\Tr$.




\begin{figure}[ht!] 
\centering
\begin{tikzpicture}[->,>=stealth', auto, node distance=2cm and 2cm, main node/.style={}]
  \node[main node] (Az) at (4,7) {$\langle A : z \rangle , \mathbf{t}$};
  \node[main node] (Bspz) at (0.5,6) {$\{B ~says~ p; B ~says~ z\}$};
  \node[main node] (Bsr) at (5,6) {$\{B ~says~ r\}$};
  \node[main node] (nBsr) at (8,6) {$\{\neg B ~says~ r\}$};
  \node[main node] (Bp) at (-1,5) {$\langle B : p \rangle , \mathbf{t}$};
  \node[main node] (Bsp) at (-1,4) {$\{\}$};
  \node[main node] (Bz1) at (1.5,5) {$\langle B : z \rangle ,  \mathbf{u}$};
  \node[main node] (Csz) at (1.5,4) {$\{C ~says~ z\}$};
  \node[main node] (Cz) at (1.5,3) {$\langle C : z \rangle , \mathbf{u}$};
  \node[main node] (Bsz) at (1.5,2) {$\{\neg B ~says~ z\}$};
  \node[main node] (Bz2) at (1.5,0.5) {\begin{tabular}{c} $\langle B : z \rangle ,  \mathbf{u}$ ~ loop! \\ (over negation)\end{tabular}};
  \node[main node] (Br1) at (5,5) {$\langle B : r \rangle ,  \mathbf{f} $};
  \node[main node] (Csr) at (5,4) {$\{C ~says~ r\}$};
  \node[main node] (Cr) at (5,3) {$\langle C : r \rangle , \mathbf{f} $};
  \node[main node] (Bsr2) at (5,2) {$\{B ~says~ r\}$};
  \node[main node] (Br2) at (5,0.5) {\begin{tabular}{c} $\langle B : r \rangle , \mathbf{f}$ ~ loop! \end{tabular}};
  \node[main node] (Br3) at (8,5) {$\langle B : r \rangle , \mathbf{f} $};
  \node[main node] (Csr2) at (8,4) {$\{C ~says~ r\}$};
  \node[main node] (Cr2) at (8,3) {$\langle C : r \rangle , \mathbf{f} $};
  \node[main node] (Bsr3) at (8,2) {$\{B ~says~ r\}$};
  \node[main node] (Br4) at (8,0.5) {\begin{tabular}{c} $\langle B : r \rangle , \mathbf{f}$ ~ loop! \end{tabular}};


  \path[every node/.style={font=\sffamily\normalsize},pos=0.5, auto]
    (Az) edge   [bend right=20] node [above] {} (Bspz)
    (Az) edge   [bend left=20]  node [above] {} (Bsr)
    (Az) edge   [bend left=20]  node [above] {} (nBsr)
    (Bspz) edge  node [right] {$\mathbf{t}$} (Bp)
    (Bp) edge    node [right] {} (Bsp)
    (Bspz) edge  node [right] {$\mathbf{t}$} (Bz1)
    (Bz1) edge   node [above] {} (Csz)
    (Csz) edge   node [right] {$\mathbf{t}$} (Cz)
    (Cz) edge    node [above] {} (Bsz)
    (Bsz) edge   node [right] {$\mathbf{f}$} (Bz2)
    (Bsr) edge   node [right] {$\mathbf{t}$} (Br1)
    (Br1) edge   node [above] {} (Csr)
    (Csr) edge   node [right] {$\mathbf{t}$} (Cr)
    (Cr) edge    node [above] {} (Bsr2)
    (Bsr2) edge  node [right] {$\mathbf{t}$} (Br2)
    (nBsr) edge  node [right] {$\mathbf{f}$} (Br3)
    (Br3) edge   node [above] {} (Csr2)
    (Csr2) edge  node [right] {$\mathbf{t}$} (Cr2)
    (Cr2) edge   node [above] {} (Bsr3)
    (Bsr3) edge  node [right] {$\mathbf{t}$} (Br4)
  ;
\end{tikzpicture}
\caption{Query Graph}
\label{fig:graph}
\end{figure}

\end{example}




\subsection{Correctness of decision procedure}
\label{sec:relation}

The following theorem states that the result of the decision procedure is always in line with the well-founded semantics of \DACL:

\begin{theorem}
\label{thm:correspondence}
 Let $\T$ be a distributed theory, let $A$ be an agent, let let $\Q$ be a \DACL formula. When $A$'s theory $\T_A$ is queried about $\Q$, the decision procedure returns $(A \says \Q)^{\wfm(\T)}$, i.e.\ the truth value of $A \says \Q$ in the well-founded model of $\T$.
\end{theorem}

We now proceed to prove Theorem \ref{thm:correspondence}.



\subsection{Proof of Theorem \ref{thm:correspondence}}

First we need to establish that the Query Minimization Procedure (Algorithm \ref{alg:query}) really does what it is supposed to do, namely to return the set of all minimal sets of \say-literals that make the query true. In order to formalize the notion of a set of \say-literals that makes the query true, we first need the following definitions of three-valued valuations of \DACL formulas, inductive definitions and theories with respect to a set of \say-literals and a structure. These definitions are analogous to the definitions \ref{def:3valform}, \ref{def:3valID} and \ref{def:3valtheo} in Appendix A:

\begin{definition}
\label{def:1}
We inductively define a three-valued valuation of \DACL formulas with respect to a set $L$ of \say-literals and a structure $\I$ as follows:
\begin{align*}
 (P(\ttt))^{L,I} & = &&  \left\{\begin{array}{ll}
                                  \Tr & \text{if } t^I\in P^I\\
                                  \Fa & \text{if } t^I\notin P^I
                                 \end{array}\right.\\
 (\neg \varphi)^{L,I}& = &&(\varphi^{L,I})^{-1}\\
 (\varphi\land \psi)^{L,I}& = &&\glb_{{\leq_t}} (\varphi^{L,I},\psi^{L,I})\\
 (\forall x \; \varphi)^{L,I}& = &&\glb_{{\leq_t}} \{\varphi[x/d]^{L,I}\mid x \in D\}\\
 (A \says \varphi)^{L,I}& = &&\left\{\begin{array}{ll}
                                  \Tr & \text{if } t^I \in \A \text{ and } \\
                                  &\hspace{3.2mm} (A \says \varphi) \in L \\
                                  \Fa & \text{if } t^I \notin \A \text{ or } \\
                                  &\hspace{3.2mm} (\neg A \says \varphi) \in L\\
                                  \Un & \text{otherwise}
                                 \end{array}\right.
% &(P(t))^{\upws,\I}=\Tr &&\text{ iff } t^I\in P^I\\
% &(t_1=t_2)^{\upws,\I}=\Tr &&\text{ iff } t_1^\I = t_2^\I\\
% &(\varphi_1 \land \varphi_2)^{\upws,\I}=\Tr &&\text{ iff } (\varphi_1)^{\upws,\I}=\Tr\text{ and } (\varphi_2)^{\upws,\I}=\Tr\\
% &(\neg \varphi)^{\upws,\I}=\Tr &&\text{ iff } (\varphi)^{\upws,\I}=\Fa\\
% &((\forall x)\varphi)^{\upws,\I}=\Tr &&\text{ iff for each } d \in D, \; (\varphi[x/d])^{\upws,\I}=\Tr\\
% &(K_{A} \varphi)^{\upws,\I}=\Tr &&\text{ iff for each $J\in \upws_A$ }(\varphi)^(\upws,J)=\Tr
\end{align*}
\end{definition}

\begin{definition}
We define a three-valued valuation of \DACL inductive definitions with respect to a set $L$ of \say-literals and a structure $\I$ as follows:
\begin{align*}
%&(\Delta)^{\upws,I}=\Tr &&\text{ if } I=wfm_{\Delta^{\upws}}(I|_{Par(\Delta)}) \\
&\Delta^{L,I}= &&\left\{\begin{array}{ll}
                                  \Tr & \text{ if } I=wfm_{\Delta^{L}}(I|_{Par(\Delta)}) \\
                                  \Fa & \text{ if } I\not\geq_p wfm_{\Delta^{L}}(I|_{Par(\Delta)}) \\
                                  \Un & \text{otherwise}
                                 \end{array}\right.
\end{align*}
where
$\Delta^L$ is the definition $\Delta$ with every formula $A \says \varphi$ replaced by $\Tr$, $\Fa$ or $\Un$, according to whether $(A \says \varphi) \in L$, $(\neg A \says \varphi) \in L$ or neither of them is in $L$.
\end{definition}

\begin{definition}
\label{def:3}
We define a three-valued valuation of \DACL theories with respect to a distributed belief pair L and a structure $\I$ as follows:
$$T^{L,I} := \glb_{\leq_t} (\{\phi^{L,I}|\phi \in T\} \cup \{\Delta^{L,I}|\Delta \in T\})$$
\end{definition}

Now we can define what it means for a set $L$ of \say-literals to make true a formula:

\begin{definition}
\label{def:4}
 Let $L$ be a set of \say-literals, let $\phi$ be a \DACL formula and let $\T$ be a \DACL theory. Then we say that $L$ \emph{makes $\phi$ true relative to $T$} iff for every structure $I$ such that $T^{L,I} \neq \Fa$ we have $\phi^{L,I} = \Tr$.
\end{definition}

The following lemma states that the Query Minimization Procedure (Algorithm \ref{alg:query}) really does what it is supposed to do:

\begin{lemma}
\label{lem:minimization}
 Let $T$ be a \DACL theory and let $\alpha$ be a \DACL formula. The set $\mathbb{L}$ returned by \textsf{Query\_{}Minimization\_{}Procedure}$(T,\alpha)$ is
 \begin{align*}
 \{L \;|\; &L \text{ is minimal (under set inclusion) among the sets $L'$ of}\\
 &\text{\say-literals that make $\alpha$ true with respect to $T$}\}
 \end{align*}
\end{lemma}

\begin{proof}
 For proving this lemma, we need to show that $L \in \mathbb{L}$ iff $L$ is a minimal set that makes $\alpha$ true with respect to $T$.

 First suppose $L \in \mathbb{L}$.
 %TODO after submission: Explain this step a bit more.
 %Then $L=\beta(S_{min}[A^{says}])$, where $S_{min} =$ min\_incons($\mathcal{T}^\prime$, $\left. S^s \right|_{A^{\says} \cup \ q}$, $\{q\}$)
 Then by the definition of Algorithm \ref{alg:query}, $\beta$ and min\_{}incons, $L$ is a minimal set such that $\mathcal{T}^\prime \cup \{p^-_{A\_\says\_\phi} \;|\; (A \says \phi) \in L\} \cup \{\neg p^+_{A\_\says\_\phi} \;|\; (\neg A \says \phi) \in L\}  \cup \{q\} \models \bot$. Hence $L$ is a minimal set such that $\mathcal{T} \cup \{p^-_{A\_\says\_\phi} \;|\; (A \says \phi) \in L\} \cup \{\neg p^+_{A\_\says\_\phi} \;|\; (\neg A \says \phi) \in L\} \models \alpha$. So by Definitions \ref{def:1}, \ref{def:3} and \ref{def:4} above, $L$ is a minimal set that makes $\alpha$ true with respect to $T$, as required.

 Conversely, suppose $L$ is a minimal set that makes $\alpha$ true with respect to $T$. Define $S$ to be the partial structure that makes $q$ true, makes $p^-_{A\_\says\_\phi}$ true whenever $(A \says \phi) \in L$, that makes $p^+_{A\_\says\_\phi}$ false whenever $(\neg A \says \phi) \in L$, and that is undefined on all other symbols.
 %TODO after submission: Explain this step a bit more.
 Then applying lines 4-6 of Algorithm \ref{alg:query} to this structure $S$ leads to $L$ being added to $\mathbb{L}$, as required.

\end{proof}

Let $\bot$ denote the DPWS that represents the lack of knowledge, i.e. in which every agent's possible world structure is the set of all structures over domain $D$ and vocabulary $\Sigma$. Let $\top$ denote the DPWS that represent inconsistent knowledge, i.e. in which every agent's possible world structure is the empty set.

The well-founded model of $\T$ is the $\leq_p$-least fixpoint of $S_\T$. When the domain is finite, as we are assuming when applying the decision procedure, there is a natural number $n$ such that $\wfm(\T) = (S_\T)^n(\bot,\top)$. In other words, the well-founded model can be computed by a finite number of application of $S_\T$ to $(\bot,\top)$, until a fixpoint is reached.

The steps in the decision procedure defined in section \ref{sec:query} do not directly correspond to the steps in the computation of the well-founded model by a finite number of application of $S_\T$ to $(\bot,\top)$. In order to prove that the two computations nevertheless always yield the same result, we first define a decision procedure that resembles the decision procedure defined in section \ref{sec:query}, but whose steps correspond more directly to the iterative application of $S_\T$ to $(\bot,\top)$. We call this auxiliary decision procedure the \emph{$S_\T$-based decision procedure}. So we prove Theorem \ref{thm:correspondence} by proving two things:
\begin{itemize}
 \item The decision procedure defined in section \ref{sec:query} is equivalent to the $S_\T$-based decision procedure.
 \item  When $A$'s theory $\T_A$ is queried about $\Q$, the $S_\T$-based decision procedure returns \textsf{yes} iff $(A \says \Q)^{\wfm(\T)} = \Tr$.
\end{itemize}

At this point the reader may wonder why we don't directly use the $S_\T$-based decision procedure as our decision procedure for the well-founded semantics. There are two reasons: The decision procedure defined in section \ref{sec:query} is more efficient, and it is better at minimizing communication between the different agents' theories, which is a relevant feature for the access control application we have in mind.

In the definition of the $S_\T$-based decision procedure, we use a \emph{query graph} as defined in section \ref{sec:query}. Unlike the query graph produced in the decision procedure from section \ref{sec:query}, the labelling of the query vertices in the query graph produced by the $S_\T$-based decision procedure are unique, i.e. there are no two distinct query vertex with the same labelling $k:\phi$.

% \begin{definition}
% \label{def:query graph}
% A \emph{query graph} is a labelled directed graph with two kinds of vertices and two kinds of edges:
%  \begin{itemize}
%   \item The first kind of vertices are the \emph{query vertices}. Each query vertex is labelled by a directed query of the form $k:\phi$, where $k$ is the principal whose theory is being queried and $\phi$ is the formula representing the query, as well as by a truth value in $\{\Tr,\Fa,\Un\}$, which represents the currently active valuation of the query at any moment during the execution of the decision procedure.
%   \item The second kind of vertices are the \emph{\say-literal set vertices}. Each \say-literal set vertex is labelled by a set of \say-literals, i.e.\ formulas of the form $k \says \phi$ or $\neg k \says \phi$.
%   \item The first kind of edges are unlabelled edges going from a query vertex to a \say-literal set vertex. The intended meaning of such an unlabelled edge from $k:\Q$ to the \say-literal set $L$ is that one way of making $\Q$ true in $k$'s theory is to make all \say-literals in $L$ true.
%   \item The second kind of edged are edges labelled by $\Tr$ or $\Fa$, goinf from a \say-literal set vertex to a query vertex. The intended meaning of such an edge labelled by $\Tr$ or $\Fa$ and going from the \say-literal set $L$ to the query $k:\Q$ is that $L$ contains the literal $k \says \Q$ or the literal $\neg k \says \Q$ respectively.
%  \end{itemize}
% \end{definition}

There is a direct correspondence between distributed belief pairs and certain truth-value labelling of the query vertices in a query graph:

\begin{definition}
 Let $G$ be a query graph. Let \ubp be a distributed belief pair. We say that the truth-value labelling of the query vertices of $G$ \emph{corresponds to} \ubp iff for each query vertex $k:\phi$ in $G$, the truth-value with which this vertex is labelled is $(k \says \phi)^\ubp$.
\end{definition}

Note that there are truth-labellings of the query vertices that do not correspond to any distributed belief pair. We call a truth-labelling of the query vertices \emph{good} iff it corresponds to some distributed belief pair.

The $S_\T$-based decision procedure works by first producing a query graph and then iteratively modifying the truth-value labelling of the query vertices. We need to ensure that after each iteration of this iterative modification, the truth-value labelling of the query vertices is good. However, there are intermediate steps within each iteration which lead to a bad labelling of the query vertices. In order to get back to a good labelling, we apply the changes defined by Algorithm \ref{alg:make good}.

\begin{algorithm}[h!t]
\caption{\textsf{Make labelling of query vertices good} \label{alg:make good}}
\begin{algorithmic}[1]
\REQUIRE{query graph $G$}
\ENSURE{modified query graph $G$}
\WHILE{there is a $\Un$-labelled query vertex $k:\phi$ in $G$ such that replacing \say-atoms in $\phi$ corresponding to $\Tr$- or $\Fa$-labelled query vertices by $\Tr$ and $\Fa$ respectively makes $\phi$ a tautology}
  \STATE{change the $\Un$-label in each such query vertex in $G$ by $\Tr$}
\ENDWHILE
\WHILE{there is a $\Fa$-labelled query vertex $k:\phi$ in $G$ such that replacing \say-atoms in $\phi$ corresponding to $\Un$-, $\Tr$- or $\Fa$-labelled query vertices by $\Tr$ or $\Fa$, $\Tr$ and $\Fa$ respectively makes $\phi$ a tautology}
  \STATE{change the $\Fa$-label in each such query vertex in $G$ by $\Un$}
\ENDWHILE
\RETURN{$G$}
\end{algorithmic}
\end{algorithm}

% It is easy to see that the output of Algorithm \ref{alg:make good} is the least precise (i.e.\ $\Un$-maximizing) good labelling of query vertices that is more precise than the input labelling.

In order to define the $S_\T$-based decision procedure, we furthermore need the following two definitions:

\begin{definition}
In a query graph, a \say-literal set vertex $L$ is defined to be \emph{satisfied} if for every $\Tr$-labelled edge from $L$ to a query vertex, the query vertex is labelled by $\Tr$, and for every $\Fa$-labelled edge from $L$ to a query vertex, the query vertex is labelled $\Fa$.
\end{definition}

\begin{definition}
In a query graph, a \say-literal set vertex $L$ is defined to be \emph{potentially satisfied} if for every $\Tr$-labelled edge from $L$ to a query vertex, the query vertex is labelled by $\Tr$ or $\Un$, and for every $\Fa$-labelled edge from $L$ to a query vertex, the query vertex is labelled $\Fa$ or $\Un$.
\end{definition}

The definition of the $S_\T$-based decision procedure is given by the pseudo-code under Algorithm \ref{alg:ST-based}. Here is an informal explanation of this definition:
\begin{itemize}
 \item First (lines 1-20) produce a query graph $G$ without truth-value label on query vertices by iteratively applying the query minimization procedure from Section \ref{sec:query} to the main query $A_\Q$, to its subqueries, their subqueries etc., adding vertices and edges to the graph in line with the informal meaning of the vertices and edges given in Definition \ref{def:query graph} above.
%  \begin{enumerate}
%   \item Make a query vertex labelled by $A:\Q$.
%   \item Assign the value $A$ to the variable $k$.
%   \item Assign the value $\Q$ to the variable $\phi$
%   \item Apply the query minimization procedure to $\T_k$ and $\phi$. The output is a set of sets of \say-literals.
%   \item For each set $L$ of \say-literals in this set, do:
%   make a \say-literal set vertex labelled by $L$, if there does not already exist such a vertex, and make an edge from the query vertex $k:\phi$ to $L$.
%  \end{enumerate}
 \item Each query vertex in $G$ is labelled $\Un$ (line 21).
 \item Next (lines 22-36) we iteratively turn some of the $\Un$-labels on queries into $\Tr$-labels and $\Fa$-labels. At each step of this iteration, we separately calculate which $\Un$-labels to change to $\Tr$ and which $\Un$-labels to turn to $\Fa$ as follows:
 \begin{enumerate}
  \item In order to calculate which $\Un$-labels to change to $\Tr$, we recursively do the following (lines 25-27): When there is an edge from a query vertex labelled $\Un$ to a satisfied \say-literal set, change the label of the query vertex to $\Tr$. Then make the labelling of the query vertices good. (All the queries whose labels change from $\Un$ to $\Tr$ in this recursive procedure are changed to $\Tr$ in $G$ in line 33.)
  \item In order to calculate which $\Un$-labels to change to $\Fa$, we first change the labelling of all $\Un$-labelled queries to $\Fa$ (line 29) and then recursively do the following (lines 30-32): When there is an edge from a query vertex labelled $\Un$ to a dissatisfied \say-literal set, change the label of the query vertex to $\Un$. Then make the labelling of the query vertices good. (All the queries whose labels stay $\Fa$ in this recursive procedure are changed to $\Fa$ in $G$ in line 34.)
 \end{enumerate}
 \item Finally, we return the truth-value by which the query vertex of the main query $A:\Q$ is labelled in $G$ (lines 37-38).
\end{itemize}


\begin{algorithm}[h!t]
\caption{\textsf{$S_\T$-based decision procedure} \label{alg:ST-based}}
\begin{algorithmic}[1]
\REQUIRE{distributed theory $\T$, principal $A$, \DACL formula $\Q$}
\ENSURE{truth-value $V \in \{\Tr,\Fa,\Un\}$}
\STATE{$G$ := the empty graph }
\STATE{add a new query vertex $A:\Q$ to $G$}
\STATE{query\_{}stack := $\langle A:\Q \rangle$}
\WHILE{query\_{}stack $\neq \langle \rangle$}
  \STATE{$k:\phi$ := first element of query\_{}stack}
  \STATE{$\LL$ := \textsf{Query\_{}Minimization\_{}Procedure}($\T_k$,$\phi$)}
  \FOR{$L \in \LL$}
    \IF{$G$ does not contain a \say-literal set vertex $L$}
      \STATE{add a new \say-literal set vertex $L$ to $G$}
      \FOR{$l \in L$}
        \STATE{$k'$ := the principal such that $l$ is of the form $k' \says \psi$ or $\neg k' \says \psi$}
        \STATE{$\psi$ := the formula such that $l$ is of the form $k' \says \psi$ or $\neg k' \says \psi$}
        \IF{$G$ does not contain a query vertex $k':\psi$}
           \STATE{add a query vertex $k':\psi$ to $G$}
           \STATE{add $k':\psi$ to query\_{}stack}
        \ENDIF
        \IF{$l$ is $k' \says \psi$}
          \STATE{add to $G$ a new edge labelled $\Tr$ from vertex $L$ to vertex $k':\psi$}
        \ENDIF
        \IF{$l$ is $\neg k' \says \psi$}
          \STATE{add to $G$ a new edge labelled $\Fa$ from vertex $L$ to vertex $k':\psi$}
        \ENDIF
      \ENDFOR
    \ENDIF
    \STATE{add to $G$ a new edge from vertex $k:\phi$ to vertex $L$}
  \ENDFOR
\ENDWHILE
\STATE{add the label $\Un$ to all query vertices in $G$}
\STATE{finished := 0}
\WHILE{finished = 0}
  \STATE{$G_1 := G$}
  \WHILE{in $G_1$ there is a query vertex labelled by $\Un$ with an edge to a satisfied \say-literal set vertex}
    \STATE{change every $\Un$-label on a query vertex with an edge to a satisfied \say-literal set vertex to $\Tr$}
    \STATE{$G$ := \textsf{Make\_{}labelling\_{}of\_{}query\_{}vertices\_{}good($G$)}}
  \ENDWHILE
  \STATE{$G_2 := G$}
  \STATE{change every $\Un$-label on a query vertex in $G_2$ to $\Fa$}
  \WHILE{in $G_2$ there is a query vertex labelled by $\Fa$ with an edge to a potentially satisfied \say-literal set vertex}
    \STATE{change every $\Fa$-label on a query vertex with an edge to a potentially satisfied \say-literal set vertex to $\Un$}
    \STATE{$G$ := \textsf{Make\_{}labelling\_{}of\_{}query\_{}vertices\_{}good($G$)}}
  \ENDWHILE
  \STATE{in $G$, change the label on all query vertices that are labelled $\Un$ in $G$ and labelled $\Tr$ in $G_1$ into $\Tr$}
  \STATE{in $G$, change the label on all query vertices that are labelled $\Un$ in $G$ and labelled $\Fa$ in $G_2$ into $\Fa$}
  \IF{no changes were made to $G$ in the previous two lines}
    \STATE{finished := 1}
  \ENDIF
\ENDWHILE
\STATE{$V$ := the label on the query vertex $A:\Q$ in $G$}
\RETURN{$V$}
\end{algorithmic}
\end{algorithm}

%TODO: Expand the following proof sketch a bit:
We now sketch the proof of the equivalence between the $S_\T$-based decision procedure and the decision procedure defined in section \ref{sec:query}: The only fundamental difference between these two decision procedures is the loop-handling. Step 2) of the $S_\T$-based decision procedure takes care of making queries looping over $\Tr$-labelled edges false. Queries looping over $\Fa$-labelled edges will always be left undecided by the $S_\T$-based decision procedure, which corresponds to making them undecided in the decision procedure defined in section \ref{sec:query}.

We now establish that the $S_\T$-based decision procedure always gives the same result as the well-founded semantics. Note that the labelling corresponding to the distributed belief pair $(\bot,\top)$ is the labelling in which all query vertices are labelled by $\Un$. Keeping in mind that the well-founded model can be computed by a finite number of application of $S_\T$ to $(\bot,\top)$, it is now easy to see that the following lemma is sufficient to establish that the $S_\T$-based decision procedure always gives the same result as the well-founded semantics:

\begin{lemma}
Let $\T$ be a distributed theory, $A$ be a principal and $\Q$ be a \DACL formula. Let $G$ be the query graph produced by lines 1-20 of Algorithm \ref{alg:ST-based} applied to $\T$, $A$ and $\Q$. Let \ubp be a distributed belief pair. Labelling the query vertices in $G$ according to \ubp and then applying lines 24 to 34 of Algorithm \ref{alg:ST-based} to $G$ yields a labelling of the queries corresponding to $S_\T(B)$.
\end{lemma}

\begin{proof}
For proving this lemma, it is enough to prove the following four properties:
\begin{enumerate}
 \item The change in the truth-value labelling of the query vertices of $G$ in lines 26-27 of Algorithm \ref{alg:ST-based} corresponds to changing the belief pair $(\upws_1,\upws_2)$ to $(D^*_\T(\upws_1,\upws_2)_1,\upws_2)$.
 \item The change in the truth-value labelling of the query vertices of $G$ in line 28 of Algorithm \ref{alg:ST-based} corresponds to changing the belief pair $(\upws_1,\upws_2)$ to $(\upws_1,\upws_1)$.
 \item The change in the truth-value labelling of the query vertices of $G$ in line 31-31 of Algorithm \ref{alg:ST-based} corresponds to changing the belief pair $(\upws_1,\upws_2)$ to $(\upws_1,D^*_\T(\upws_1,\upws_2)_2)$.
 \item Let $\upws_1,\upws_2,\upws_3,\upws_4$ be DPWS's such that $\upws_3 \leq_K \upws_1 \leq_K \upws_4 \leq_K \upws_2$. If the query vertices are labelled $\Tr$ in correspondence with the distributed belief pair $(\upws_1,\upws_2)$, labelled $\Fa$ in correspondence with the distributed belief pair $(\upws_3,\upws_4)$, and labelled $\Un$ otherwise, the resulting labelling corresponds to the distributed belief pair $(\upws_1,\upws_4)$.
\end{enumerate}

Noting that a \say-atom satisfied by the DPWS $\upws_1$ is true according to the distributed belief pair $(\upws_1,\upws_2)$, and that a \say-atom satisfied by the DPWS $\upws_2$ is not false according to the distributed belief pair $(\upws_1,\upws_2)$, it is easy to see that Properties 2) and 4) hold.

\textbf{Proof of Property 1):} Suppose the labelling of query vertices corresponds to $(\upws_1,\upws_2)$. It is enough to show that lines 26-27 change a labelling of a query vertex $k:\phi$ from $u$ to $t$ iff $(k \says \phi)^{D^*_\T(\upws_1,\upws_2)} = \Tr$.

So first suppose that line 26 changes the labelling of $k:\phi$ from $u$ to $t$. This means that there is an edge from $k:\phi$ to a satisfied \say-literal set vertex $L$. By Lemma \ref{lem:minimization}, $L$ fixes the truth value of $\phi$ to be true relative to $\T_k$.
Since the \say-literal set vertex $L$ is satisfied under the labelling of query vertices corresponding to $(\upws_1,\upws_2)$, this means that $\phi^{(\upws_1,\upws_2),I} = \Tr$ for every structure $I$ such that $(\T_k)^{(\upws_1,\upws_2),I} \neq \Fa$. Since $(\upws_1,\upws_2) \leq_p D^*_\T(\upws_1,\upws_2)$, it follows that $\phi^{D^*_\T(\upws_1,\upws_2),I} = \Tr$ for every structure $I$ such that $(\T_k)^{(\upws_1,\upws_2),I} \neq \Fa$. By Definition \ref{def:D*}, $D^*_\T(\upws_1,\upws_2)_1 = (\T_A)^{(\upws_1,\upws_2),I} \neq \Fa \})_{A\in \A}$. So $(k \says \phi)^{D^*_\T(\upws_1,\upws_2)} = \Tr$, as required.

Now suppose that line 27 changes the labelling of $k:\phi$ from $u$ to $t$. So there is a distributed belief pair $\ubp$ with $(\upws_1,\upws_2) \leq_p \ubp \leq_p D^*_\T(\upws_1,\upws_2)$ such that replacing \says-atoms in $\phi$ by their truth values under $\ubp$ makes $\phi$ a tautology. In other words, $\phi^{\ubp,I} = \Tr$ for any structure $I$, i.e. $\phi^{D^*_\T(\upws_1,\upws_2),I} = \Tr$ for any structure $I$, i.e. $(k \says \phi)^{D^*_\T(\upws_1,\upws_2)} = \Tr$ ,as required.

Now suppose that $(k \says \phi)^{D^*_\T(\upws_1,\upws_2)} = \Tr$. Then $\phi^{D^*_\T(\upws_1,\upws_2),I} = \Tr$ for every $I$ such that $(\T_k)^{(\upws_1,\upws_2),I} \neq \Fa$.
%TODO: Improve the following proof steps:
Now there are two different cases: Either $\phi^{\upws_1,\upws_2),I} = \Tr$ for every $I$ such that $(\T_k)^{(\upws_1,\upws_2),I} \neq \Fa$, or $\phi^{D^*_\T(\upws_1,\upws_2),I} = \Tr$ for every structure $I$. In the first case, line 26 changes the labelling of $k:\phi$ from $u$ to $t$. In the second case, line 27 changes the labelling of $k:\phi$ from $u$ to $t$.

Property 2) can be proven in a similar way as property 1).
\end{proof}

This completes the proof of Theorem \ref{thm:correspondence}.



==> idp-latex/idp-latex-no-theorem.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex-no-theorem}
% \usepackage{import}
\providecommand\idplatexdir{idp-latex}

\input{\idplatexdir/includes-no-theorems}
\input{\idplatexdir/common-citations}
% \subimport{idp-latex/}{includes-no-theorems}
% \subimport{idp-latex/}{common-citations}




%The following are directives for LaTeX editors that collect ``included files'' to autocomplete macros etcetera
\ignore{
\include{includes-no-theorems}
\include{common-citations}
}


==> idp-latex/idp-listings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             Stuff for writing IDP source code with coloring              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\usepackage[final]{listings}

	\lstdefinelanguage{idp}{
		morekeywords=[1]{query(}, %to ignore procedure calls to query
		morekeywords=[2]{namespace,vocabulary,theory,structure,procedure,term,set,formula, spec, specification,query},
		morekeywords=[3]{include,using,type,isa,contains,partial,extern,LFD,GFD,constructed,from,constraint,pred,supertype,of,subtype,define},
		morekeywords=[4]{int,float,char,string,nat},
		morekeywords=[5]{if,then,else,for,end},
		morecomment=[s]{/*}{*/},	
		morecomment=[l]{//}
	}
	\lstset{
		language=idp,
		tabsize=3,
		basicstyle=\small,
		frame=none,
		frame=single,
		showstringspaces=false,
		breaklines = true,
		alsoletter=(,
		commentstyle=\commentstyle,
		keywordstyle=[1],
		keywordstyle=[2]\color{BrickRed}\bfseries,
		keywordstyle=[3]\color{OliveGreen}\bfseries,
		keywordstyle=[4]\color{Blue}\bfseries,
		keywordstyle=[5]\color{Violet}\bfseries,
		literate={~} {$\sim$}{1}
	}
	\newcommand{\code}[1]{\texttt{#1}}

